Orthrus: Accelerating Multi-BFT Consensus through Concurrent Partial Ordering of Transactions (Extended Version)

Multi-Byzantine Fault Tolerant (Multi-BFT) consensus allows multiple consensus instances to run in parallel, resolving the leader bottleneck problem inherent in classic BFT consensus. However, the global ordering of Multi-BFT consensus enforces a strict serialized sequence of transactions, imposing additional confirmation latency and also limiting concurrency. In this paper, we introduce Orthrus, a Multi-BFT protocol that accelerates transaction confirmation through partial ordering while reserving global ordering for transactions requiring stricter sequencing. To this end, Orthrus strategically partitions transactions to maximize concurrency and ensure consistency. Additionally, it incorporates an escrow mechanism to manage interactions between partially and globally ordered transactions. We evaluated Orthrus through extensive experiments in realistic settings, deploying 128 replicas in WAN and LAN environments. Our findings demonstrate latency reductions of up to 87% in WAN compared to existing Multi-BFT protocols.

==> annotations.tex <==
\usepackage{ifthen}
%\usepackage[normalem]{ulem} % for \sout
%\usepackage{xcolor}
%\usepackage{amssymb}
%\newcommand{\ra}{$\rightarrow$}
\newboolean{showedits}
\setboolean{showedits}{true} % toggle to show or hide edits
% \setboolean{showedits}{false} % toggle to show or hide edits

\ifthenelse{\boolean{showedits}}
{
	\newcommand{\ugh}[1]{\textcolor{red}{\uwave{#1}}} % please rephrase
	\newcommand{\ins}[1]{\textcolor{blue}{\uline{#1}}} % please insert
	\newcommand{\del}[1]{\textcolor{red}{\sout{#1}}} % please delete
	\newcommand{\chg}[2]{\textcolor{red}{\sout{#1}}{\ra}\textcolor{blue}{\uline{#2}}} % please change
}{
	\newcommand{\ugh}[1]{#1} % please rephrase
	\newcommand{\ins}[1]{#1} % please insert
	\newcommand{\del}[1]{} % please delete
	\newcommand{\ch}[2]{#2}
}

\newcommand{\cbox}[2][yellow]{%
  \colorbox{#1}{\parbox{\dimexpr\linewidth-2\fboxsep}{\strut #2\strut}}%
}

\newboolean{showcomments}
\setboolean{showcomments}{true}
% \setboolean{showcomments}{false}
\newcommand{\id}[1]{$-$Id: scgPaper.tex 32478 2010-04-29 09:11:32Z oscar $-$}
%\newcommand{\yellowbox}[1]{\fcolorbox{gray}{yellow}{\bfseries\sffamily\scriptsize\parbox{\dimexpr\linewidth-2\fboxsep}{\strut #1\strut}}}
\newcommand{\yellowbox}[1]{\\ \fcolorbox{gray}{yellow}{\parbox{\dimexpr\linewidth-2\fboxsep}{\strut #1\strut}}}
\newcommand{\triangles}[1]{{\sf\small$\blacktriangleright$\textit{#1}$\blacktriangleleft$}}
\ifthenelse{\boolean{showcomments}}
%{\newcommand{\nb}[2]{{\yellowbox{#1}\triangles{#2}}}
{\newcommand{\nbc}[3]{
 {\colorbox{#3}{\bfseries\sffamily\scriptsize\textcolor{white}{#1}}}
 {\textcolor{#3}{\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}}}
 \newcommand{\version}{\emph{\scriptsize\id}}}
{\newcommand{\nbc}[3]{}
 \renewcommand{\ugh}[1]{#1} % please rephrase
 \renewcommand{\ins}[1]{#1} % please insert
 \renewcommand{\del}[1]{} % please delete
 \renewcommand{\chg}[2]{#2} % please change
 \newcommand{\version}{}}
 \definecolor{darkyellow}{RGB}{255, 222, 9}
 \newcommand{\nb}[2]{{\yellowbox{#1 \triangles{#2}}}}
%\newcommand{\nb}[2]{\nbc{\parbox{\dimexpr\linewidth-2\fboxsep}{\strut #1\strut}}{#2}{orange}}

\definecolor{ibcolor}{rgb}{0.4,0.6,0.2}
\definecolor{ascolor}{rgb}{0,0.5,0.9}

\definecolor{bocolor}{rgb}{0.6,0.9,0.2}
\definecolor{jrcolor}{rgb}{0.5,0,0.5}
\definecolor{nrcolor}{rgb}{0.4,0.1,0.3}
\definecolor{hkcolor}{rgb}{1.0,0.5,0.3}
\definecolor{tdcolor}{rgb}{1.0,0,0}

\newcommand\iv[1]{\nbc{IB}{#1}{ibcolor}}
\newcommand\arsj[1]{\nbc{AS}{#1}{ascolor}}
\newcommand\don[1]{\nbc{DB}{#1}{nrcolor}}
\newcommand\vs[1]{\nbc{VS}{#1}{jrcolor}}
\newcommand\dm[1]{\nbc{DM}{#1}{bocolor}}
\newcommand\mk[1]{\nbc{MK}{#1}{hkcolor}}
\newcommand\todo[1]{\nbc{TODO}{#1}{tdcolor}}

